Online partial evaluation of sheet-defined functions

We present a spreadsheet implementation, extended with sheet-defined functions, that allows users to define functions using only standard spreadsheet concepts such as cells, formulas and references, requiring no new syntax. This implements an idea proposed by Peyton-Jones and others. As the main contribution of this paper, we then show how to add an online partial evaluator for such sheet-defined functions. The result is a higher-order functional language that is dynamically typed, in keeping with spreadsheet traditions, and an interactive platform for function definition and function specialization. We describe an implementation of these ideas, present some performance data from microbenchmarks, and outline desirable improvements and extensions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{136}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.10}{10.4204/EPTCS.129.10}}
\pdfoutput=1

